CardioID: Mitigating the Effects of Irregular Cardiac Signals for Biometric Identification

Cardiac patterns are being used to obtain hard-to-forge biometric signatures and have led to high accuracy in state-of-the-art (SoA) identification applications. However, this performance is obtained under controlled scenarios where cardiac signals maintain a relatively uniform pattern, facilitating the identification process. In this work, we analyze cardiac signals collected in more realistic (uncontrolled) scenarios and show that their high signal variability (i.e., irregularity) makes it harder to obtain stable and distinct user features. Furthermore, SoA usually fails to identify specific groups of users, rendering existing identification methods futile in uncontrolled scenarios. To solve these problems, we propose a framework with three novel properties. First, we design an adaptive method that achieves stable and distinct features by tailoring the filtering spectrum to each user. Second, we show that users can have multiple cardiac morphologies, offering us a much bigger pool of cardiac signals and users compared to SoA. Third, we overcome other distortion effects present in authentication applications with a multi-cluster approach and the Mahalanobis distance. Our evaluation shows that the average balanced accuracy (BAC) of SoA drops from above 90% in controlled scenarios to 75% in uncontrolled ones, while our method maintains an average BAC above 90% in uncontrolled scenarios.

==> sec/system_overview.tex <==
\subsection{Applications, metrics and system overview} 
\label{subsec:principle}

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figure/Cluster_analysis.pdf}
\caption{Key principles for identification: 1) minimize the variance of clusters and 2) maximize the distance between clusters.}
\label{fig:classification_principle}
\end{figure}

Our system analyzes the performance of two different applications: identification and authentication. Until now we have been using the term \textit{identification} to refer to both, but there is a key difference between them. In identification, the population size is \textit{known} and the training phase requires gathering data from \textit{all} individuals. In authentication, the population size is \textit{unknown} and the training phase \textit{only} gathers data from the user of interest. Performing authentication is more challenging than performing classification. \tocheck{No study in the SoA has tested its methods with both application, they only focus on one (usually classification)}\todo{Is this statement true?}. Our study analyzes both. 

Independently of the targeted application, performing identification with PPG signals requires tackling two main challenges, as shown in~\autoref{fig:classification_principle}.

\begin{itemize}
    \item \textit{\textbf{Challenge 1}: reduce intra-cluster variance.} We need cardiac cycles that are as homogeneous as possible for the same individual, in order to obtain stable features.
    \item \textit{\textbf{Challenge 2}: increase inter-cluster distance.} We need cardiac cycles that are as different as possible among individuals, in order to define clear identification boundaries.
\end{itemize} 

For the reminder of the paper we will use the term \textit{morphology} to refer to the shape of a cardiac cycle, and \textit{stable morphology} to refer to cardiac cycles that have (i) the same numbers of peaks and valleys, and (ii) a small signal variance. For example, \autoref{fig:controlled_ppg} depicts a stable morphology with two peaks and {three valleys}. When signals are gathered in an uncontrolled environment, attaining distinct and stable morphologies for each user becomes significantly more complex.


\add[Eric]{should we elaborate the evaluation metrics,like BAC, TPR or FPR?}

Our system has three main phases: filtering, feature extraction and testing. For the input data, we consider two types of sensors: PPG sensor (data obtained from an open data set) and smartphone (data collected locally with the embedded flashlight and camera). Also, 

% \begin{figure*}[hbt!]
% \centering
% \includegraphics[width=\linewidth]{figure/System_design.pdf}
% \caption{The system overview}
% \label{fig:system_design}
% \end{figure*}

% Existing cardiac applications using the smartphone camera only measure the user's heartbeat. While our system aims at identifying people. The system flow is shown in Fig.~\ref{fig:system_design}. The system consists of 3 major phases:
% 1) morphology stabilization. 2) feature extraction. 3) identification.

% Thus, the following of this paper will be organized in terms of these phases.


%On the left of Fig.\ref{fig:classification_principle}\todo{This figure needs to change. 1) Why show the green cluster? Show only blue and red and don't overlap the periods (bottom right figures) 2) The image is not sharp}, we can see there are three clusters. The purpose of all authentication and identification systems is to have high classification accuracy. In order to achieve that, there are two essences: 1. samples inside the cluster are compact. 2. distances between clusters are far. 

%The first essence means the variance of a cluster should be small. In our case, this means that the morphology of one subject, which is the overall signal shape, should be stable as shown on the top right of Fig.\ref{fig:classification_principle}. From this picture, all periods are highly overlapped with each other to form a compact morphology. 
%The compact morphology consists of two levels. First, the macro morphology, which is the numbers of peaks and troughs in each period, should be constant. Second, The micro morphology, which is locations of peaks and troughs in all periods, should be stable.
%The first essence is the foundation of the system. If a system can compact each cluster, the distances between clusters will become larger. This is the reason why the controlled data set $\mathcal{C}$ can perform \textbf{nearly perfect} identification and authentication. The periods they collect are from a compact morphology. 


%The second essence can be interpreted as the bottom right of Fig.\ref{fig:classification_principle} in our case. The morphologies from two different subjects are distinguishing. The macro morphology is different for both subjects. The micro morphology is different too. 

%Our system will be designed according to these two essences.


%The crux of the problem is that an irregular PPG signal (i) makes it more difficult to obtain a unique set of features to identify a single individual, and (ii) creates irregular clusters in the feature space, making it harder to create classification boundaries to differentiate among various individuals. 

==> table/Abbreviation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h!]
\centering
\caption{A list of abbreviation in our paper.(The Red abbreviation only use once.)}
\vspace{-3mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{llllllll}
{\color[HTML]{FE0000} AUC} & Area Under Curve                                                                         & BAC                         & Balanced Accuracy                                                                 & {\color[HTML]{FE0000} BIRCH}  & \begin{tabular}[c]{@{}l@{}}Balanced Iterative Reducing and \\ Clustering using Hierarchies\end{tabular}                & {\color[HTML]{FE0000} CLIQUE} & Clustering in QUEst                                                                           \\
CTE                        & Cross Track Error                                                                        & {\color[HTML]{FE0000} CWT}  & Continuous Wavelet Transform                                                      & {\color[HTML]{FE0000} DBSCAN} & \begin{tabular}[c]{@{}l@{}}Density-Based Spatial Clustering \\ of Applications with Noise\end{tabular}                 & {\color[HTML]{FE0000} DWT}    & Discrete Wavelet Tranform                                                                     \\
ECG                        & Electrocardiogram                                                                        & EER                         & Equal Error Rate                                                                  & {\color[HTML]{FE0000} FFT}    & Fast Fourier Transform                                                                                                 & {\color[HTML]{FE0000} FPS}    & Frames Per Second                                                                             \\
{\color[HTML]{FE0000} ISO} & \begin{tabular}[c]{@{}l@{}}International Organization\\ for Standardization\end{tabular} & {\color[HTML]{000000} K-NN} & K-Nearest Neighbors                                                               & {\color[HTML]{000000} LDA}    & Linear Discriminant Analysis                                                                                           & {\color[HTML]{FE0000} LED}    & Light Emitting Diode                                                                          \\
{\color[HTML]{FE0000} LLE} & Local Linear Embedding                                                                   & Mahal                       & \begin{tabular}[c]{@{}l@{}}Mahalanobis variant for\\ baseline system\end{tabular} & {\color[HTML]{000000} MC}     & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Morphology Classification variant\\ for baseline system\end{tabular}} & {\color[HTML]{000000} MS}     & \begin{tabular}[c]{@{}l@{}}Morphology Stablization variant\\ for baseline system\end{tabular} \\
{\color[HTML]{FE0000} NMF} & Non-negative matrix Factor                                                               & NN                          & Neural Network                                                                    & {\color[HTML]{FE0000} OPTICS} & \begin{tabular}[c]{@{}l@{}}Ordering Points To Identify the\\ Clustering Structure\end{tabular}                         & PCA                           & Principal Component Analysis                                                                  \\
PPG                        & Photoplethysmogram                                                                       & {\color[HTML]{FE0000} RD}   & Recording Duration                                                                & {\color[HTML]{FE0000} SVM}    & Support Vector Machine                                                                                                 & {\color[HTML]{FE0000} t-SNE}  & \begin{tabular}[c]{@{}l@{}}t-Distribution Stochastic \\ Neighbour Embedding\end{tabular}      \\
WaveClust                  & Wavelet-based Clustering                                                                 &                             &                                                                                   &                               &                                                                                                                        &                               &                                                                                              
\end{tabular}
}
\end{table}

==> table/MIMIC_dataset_period_num.tex <==
\begin{table}[t]
\centering
\caption{Percentage of detectable subjects and periods in the MIMIC-III dataset.}
\label{Tab:MIMIC_periods}
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{MIMIC-III} & \textbf{Signal variance} & \textbf{2} & \textbf{4} & \textbf{6}    & \textbf{All}  \\ \hline
\multirow{2}{*}{\cite{kavsaouglu2014novel}} & Subject \%      & 70   & 90   & 90   & 90   \\ \cline{2-6} 
                         & Period \%       & 28.4 & 53.1 & 60.6 & 66.3 \\ \hline
\multirow{2}{*}{\cite{liu2019cardiocam}} & Subject \%      & 40   & 80   & 80   & 80   \\ \cline{2-6} 
                         & Period \%       & 11   & 29.3 & 34.2 & 37.4 \\ \hline
\multirow{2}{*}{MS}      & Subject \%      & 70   & 80   & 90   & 90   \\ \cline{2-6} 
                         & Period \%       & 8.6  & 20.7 & 26.3 & 31.8 \\ \hline
\multirow{2}{*}{MC}      & Subject \%      & 80   & 100  & 100  & 100  \\ \cline{2-6} 
                         & Period \%       & 25.2 & 59.8 & 77.9 & 97.1 \\ \hline
\end{tabular}

\end{table}

% & \textbf{\begin{tabular}[c]{@{}c@{}}Signal \\ variance\end{tabular}} & \textbf{2} & \textbf{4} & \textbf{6} & \textbf{All} 

==> table/MIMIC_situation.tex <==
\begin{table*}[t]
\centering
\caption{Information of the subjects in the MIMIC-III dataset.}
\label{Tab:MIMIC_subjects}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|c|c|c|c|c|c|l|}
\hline
\begin{tabular}[c]{@{}l@{}} \textbf{Subject ID} \end{tabular} & \textbf{Gender} & \textbf{Ethnicity} & \begin{tabular}[c]{@{}l@{}} \textbf{Training data} \\ \textbf{collection time} \end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Testing data} \\ \textbf{collection time} \end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Interval (hours)}\end{tabular} & \textbf{Disease}                        \\ \hline
10045      & F      & W         & 23:32                                                                   & 9:31                                                                   & 10       & Fever                          \\ \hline
10083      & F      & W         & 12:28                                                                   & 23:28                                                                  & 11       & Hypetension                    \\ \hline
10124      & F      & Jewish    & 9:34                                                                    & 18:05                                                                  & 9        & Congestive heart failure \\ \hline
41976      & M      & Hispan    & 23:18                                                                   & 20:50                                                                  & 21       & Pneumonia                      \\ \hline
42033      & F      & W         & 17:29                                                                   & 13:38                                                                  & 20       & Shortness of breath            \\ \hline
42199      & F      & W         & 12:41                                                                   & 20:09                                                                  & 8        & Chest pain                     \\ \hline
42302      & F      & W         & 12:42                                                                   & 19:32                                                                  & 7        & Asthma COPD Flare              \\ \hline
42367      & F      & W         & 11:59                                                                   & 19:59                                                                  & 8        & Seizure; status epilepticus    \\ \hline
43798      & M      & W         & 18:27                                                                   & 5:34                                                                   & 11       & Esophageal CA/SDA              \\ \hline
43827      & F      & Unknow    & 13:29                                                                   & 20:47                                                                  & 7        & MI congestive heart failure                         \\ \hline
\end{tabular}

\end{table*}

==> table/background_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htb]
\begin{tabular}{|c|c|c|c|c|c|l|}
\hline
\multirow{2}{*}{Category} & \multirow{2}{*}{Signal}& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unique \&\\ ubiquitous\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}High security\\ level\end{tabular}}& \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}No \\additional\\ cost\end{tabular}}} \\ \cline{4-5}
& & & \begin{tabular}[c]{@{}c@{}}Obtain\\ \& forge\end{tabular} & \begin{tabular}[c]{@{}c@{}}Status\\ check\end{tabular} & \multicolumn{2}{c|}{} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}External\\ geometric\end{tabular}} & Fingerprint  &5 &1 &0 &\multicolumn{2}{c|}{0} \\ \cline{2-7} 
& \begin{tabular}[c]{@{}c@{}}Face\\ recognition\end{tabular} &5 &1 &0 &\multicolumn{2}{c|}{0} \\ \cline{2-7} 
& Iris &5 &3 &0 &\multicolumn{2}{c|}{0} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Internal\\ geometric\end{tabular}} & HBC &5 &3 &0 & \multicolumn{2}{c|}{0} \\ \cline{2-7} 
& \begin{tabular}[c]{@{}c@{}}Vein\\ pattern\end{tabular} &5 &4 &0 & \multicolumn{2}{c|}{0} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Internal\\ dynamic\end{tabular}}   & ECG &5 &5 &5 & \multicolumn{2}{c|}{0} \\ \cline{2-7} 
& PPG &5 &5 &5 & \multicolumn{2}{c|}{0}\\ \hline
\end{tabular}
\end{table}

==> table/comparison_soa.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        & 
        \multicolumn{2}{c|}{Identification~\cite{kavsaouglu2014novel}} &  \multicolumn{2}{c|}{Authentication~\cite{liu2019cardiocam}} \\
        &
        $\mathcal{C}$ & 
        $\mathcal{U}$ & 
        $\mathcal{C}$ & 
        $\mathcal{U}$ \\ 
        \hline
        precision & 88.9\% & 68.7\% & 97.2\% & 83.2\%\\
        \hline
        recall    & 90.6\% & 71.2\% & 92.9\% & 71.5\%\\
        \hline
    \end{tabular}
    \caption{Performance of SoA with controlled ($\mathcal{C}$) and uncontrolled ($\mathcal{U}$) data sets. The signal irregularity in the uncontrolled set ($\mathcal{U}$) reduces significantly the precision and recall.}
    \label{tab:comparison_soa}
\end{table}

==> table/datasets_period_num.tex <==
\begin{table}[t]
\centering
\vspace{-2mm}
\begin{minipage}{.48\linewidth}
    \caption{Percentage of detectable subjects and periods in the pulse-oximeter dataset.}
    \vspace{-3mm}
    \label{Tab:online_periods}
    \centering
    \renewcommand{\arraystretch}{1.05}
    \normalsize
    \resizebox{.88\linewidth}{!}{
    \begin{tabular}{|l|l|r|r|r|r|}
    \hline
                                                                 & \textbf{Signal Variance} & \textbf{2}    & \textbf{4}    & \textbf{6}     & \textbf{All} \\ \hline
    \multirow{2}{*}{\cite{kavsaouglu2014novel}} & subject \%     & 82.9   & 100   & 100    & 100             \\ \cline{2-6} 
                                                & period \%      & 23.4 & 58.8 & 73.0 & 80.9           \\ \hline
    \multirow{2}{*}{\cite{liu2019cardiocam}}    & subject \%     & 68.6   & 80.0   & 82.9    & 82.9              \\ \cline{2-6} 
                                                & period \%      & 21.1 & 49.8 & 59.9  & 64.2            \\ \hline
    \multirow{2}{*}{MS}                         & subject \%     & 80.0   & 97.1   & 97.1    & 97.1              \\ \cline{2-6} 
                                                & period \%      & 15.7 & 39.5 & 48.6  & 56            \\ \hline
    \multirow{2}{*}{MC}                         & subject \%     & 85.7   & 100   & 100    & 100              \\ \cline{2-6} 
                                                & period \%      & 27.5 & 69.0 & 94.6 & 96.7           \\ \hline
    \end{tabular}}
\end{minipage}
\hfill 
\begin{minipage}{.48\linewidth}
    \caption{Percentage of detectable subjects and periods in the camera dataset.}
    \label{Tab:camera_periods}
    \vspace{-3mm}
    \centering
    \renewcommand{\arraystretch}{1.05}
    \normalsize
    \resizebox{.88\linewidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
                        & \textbf{Signal Variance} & \textbf{2}    & \textbf{4}    & \textbf{6}    & \textbf{All}   \\ \hline
    \multirow{2}{*}{\cite{kavsaouglu2014novel}} & subject \%      & 37.2 & 90.7 & 100  & 100   \\ \cline{2-6} 
                        & period \%       & 6.0  & 35.8 & 55.4 & 76.1  \\ \hline
    \multirow{2}{*}{\cite{liu2019cardiocam}} & subject \%      & 25.6 & 41.9 & 58.1 & 69.8  \\ \cline{2-6} 
                        & period \%       & 5.1  & 19.5 & 28.0 & 35.5  \\ \hline
    \multirow{2}{*}{MS} & subject \%      & 25.6 & 79.1 & 88.4 & 100 \\ \cline{2-6} 
                        & period \%       & 5.0  & 24.6 & 37.1 & 52.5  \\ \hline
    \multirow{2}{*}{MC} & subject \%      & 41.9 & 90.7 & 100  & 100   \\ \cline{2-6} 
                        & period \%       & 9.4  & 46.5 & 69.5 & 96.6  \\ \hline
    \end{tabular}}
\end{minipage}
\vspace{-3mm}
\end{table}

==> table/dimensionality_estimation.tex <==
\begin{table}[hb!]
\centering
\caption{The dimensionality estimation of feature sets in three different morphologies.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
Morphology & Feature number  & Correlation  & Nearest neighbor  & Eigenvalue & GMST\\ \hline
$h_1''(t)$  & 32    & 2.2498   & 0.26109 & 5    & 3.909\\
$h_2''(t)$  & 38    & 2.1491   & 0.20973 & 6    & 3.98\\
$h_3''(t)$  & 44    & 3.0708   & 0.16923 & 10   & 5.5841 \\ \hline
\end{tabular}
}
\label{Tab:dim_estimation}
\end{table}

==> table/motivation_bad_cam.tex <==
\begin{table}[]
\centering
\caption{The result by \cite{liu2019cardiocam} method for all signal periods.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}
\hline
          & Subject 1 & Subject 2 & Subject 3 & Subject 4 & Subject 5 & Subject 6 \\ \hline
Precision & 0.79065   & 0.597701  & 0.67354   & 0.981618  & 0.997085  & 0.594684  \\ 
Recall    & 0.649416  & 0.464286  & 0.712727  & 0.610984  & 0.669276  & 0.391685  \\ \hline
\end{tabular}
}
\label{Tab:bad_cam}
\end{table}

==> table/motivation_bad_journal.tex <==
\begin{table}[]
\centering
\caption{The result by \cite{kavsaouglu2014novel} method for all signal periods.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}
\hline
          & Subject 1 & Subject 2 & Subject 3 & Subject 4 & Subject 5 & Subject 6 \\ \hline
Precision & 0.546269  & 0.808955  & 0.337313  & 0.913433  & 0.883582  & 0.629851  \\ 
Recall    & 0.690566  & 0.728495  & 0.520737  & 0.950311  & 0.989967  & 0.394393  \\ \hline
\end{tabular}
}
\label{Tab:bad_journal}
\end{table}

==> table/motivation_good_cam.tex <==
\begin{table}[]
\centering
\caption{The result by \cite{liu2019cardiocam} method for clean dataset.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}
\hline
          & Subject 1 & Subject 2 & Subject 3 & Subject 4 & Subject 5 & Subject 6 \\ \hline
Precision & 1         & 1         & 0.677419  & 0.944444  & 1         & 0.933333  \\ 
Recall    & 0.8       & 0.916667  & 0.875     & 1         & 0.692308  & 0.823529  \\ \hline
\end{tabular}
}
\label{Tab:good_cam}
\end{table}

==> table/motivation_good_journal.tex <==
\begin{table}[]
\centering
\caption{The result by \cite{kavsaouglu2014novel} method for clean dataset.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllllll}
\hline
          & Subject 1 & Subject 2 & Subject 3 & Subject 4 & Subject 5 & Subject 6 \\ \hline
Precision & 0.866667  & 1         & 0.6       & 1         & 0.933333  & 0.933333  \\ 
Recall    & 0.866667  & 1         & 0.9       & 1         & 1         & 0.666667  \\ \hline
\end{tabular}
}
\label{Tab:good_journal}
\end{table}

==> table/paper_dataset.tex <==
\begin{table}[]
\centering
\caption{Using subjects can be detected by \cite{liu2019cardiocam} in camera dataset, we form a new dataset called paper dataset. In this dataset, We test that the number of detectable subjects and periods can be collected. \cmq{move the caption to the top.}}
\label{tab:paper_dataset}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
                                                          & Signal variance & 2   & 4    & 6    & \textgreater{}6 \\ \hline
\multirow{2}{*}{\cite{liu2019cardiocam}} & subject \#      & 8   & 11   & 13   & 14              \\ \cline{2-6} 
                                                          & period \#       & 325 & 1198 & 1632 & 1885            \\ \hline
\multirow{2}{*}{MS}                                       & subject \#      & 7   & 10   & 12   & 14              \\ \cline{2-6} 
                                                          & period \#       & 241 & 1059 & 1556 & 2016            \\ \hline
\multirow{2}{*}{MC}                                       & subject \#      & 8   & 11   & 13   & 14              \\ \cline{2-6} 
                                                          & period \#       & 307 & 1870 & 2796 & 3766            \\ \hline
\end{tabular}

\end{table}
